Memory Classifiers: Two-stage Classification for Robustness in Machine Learning

The performance of machine learning models can significantly degrade under distribution shifts of the data. We propose a new method for classification which can improve robustness to distribution shifts, by combining expert knowledge about the ``high-level" structure of the data with standard classifiers. Specifically, we introduce two-stage classifiers called memory classifiers. First, these identify prototypical data points -- memories -- to cluster the training data. This step is based on features designed with expert guidance; for instance, for image data they can be extracted using digital image processing algorithms. Then, within each cluster, we learn local classifiers based on finer discriminating features, via standard models like deep neural networks. We establish generalization bounds for memory classifiers. We illustrate in experiments that they can improve generalization and robustness to distribution shifts on image datasets. We show improvements which push beyond standard data augmentation techniques.

==> future_experiments.tex <==
\newpage
\section{Future Experiments}
[To be deleted before submission. This section is for planning purposes only] \\ 

There seems to be a few directions we can take to improve the experimental evaluations of this paper.
\begin{itemize}
    \item Combining/comparing with other SOTA approaches which have targeted similar type of perturbations. There is this new paper (Feb-2022) \citep{noisy_mix_paper} which seems to have the best performance on Imagenet. This according to the RobustBench competition(https://robustbench.github.io/). In the same paper they show comparison with other $8-9$ types of data augmentation strategies including theirs - \textit{NoisyMix}. The set of experiments would be to combine Memory Classifiers with NoisyMix-augmentations and report our improvements. Potentially repeat the other data-augmentation techniques as well.
    
    \item There seems to be an interesting situation that arises with deep-learning for medical systems in practice, \citep{DBR-chi-paper}. This is a case study from diabetic retinopathy, where the deep learning system is trained to work on full fundus images of the eye. But, the failure rate is high for slight deviations from training set. The nurse in Thailand (the place of the case study), tried to use $2-$half images due to lack of single good quality image setting. 
    \begin{figure}[h]
        \centering
        \includegraphics[scale = 0.5]{./Figures/retinopathy}
        % \caption{}
        \label{fig:retinopathy}
    \end{figure}
    
    This is a big deviation in terms of the image space, but still classifiable by the nurse in the hospital. Deep learning systems fail here. Can we propose something similar for our experiments ? 
    
    \item \color{blue}Please feel free to add your suggestions here ! \color{black}
\end{itemize}

==> introduction.tex <==
\section{Introduction}
Modern machine learning (ML) systems have achieved extraordinary performance in a variety of domains.
%, and forms a fundamental building block for machine learning (ML). 
However, there are still significant challenges to overcome, such as interpretability, adversarial examples, and sample efficiency.
%general consensus points at a qualitative difference between human cognition and machine learning models such as deep learning. 
Infusing ML models with appropriate inductive biases may aid these challenges \citep{prior_knowledge_2, prior_knowledge_4, prior_knowledge_3}. Such useful priors are available in at least two distinct ways: as model architectures, and as manufactured examples \citep{ai_system_critic}. %An interesting anecdote about the latter, is that possible variations are augmented as additional data, to be re-acquired from the data through training.
% We propose a third avenue here, to make the prior knowledge available as a function module that can be evaluated to produce a coarse understanding of input space.
We propose a different approach, \mcs, a new learning model that relies on forming memories based on a coarsened input space in a specific way, followed by local classification based on finer features.


\textbf{Motivation.} A key challenge motivating us is to handle adversarial inputs \citep{biggio2013evasion,szegedy2013intriguing}, which are a serious roadblock limiting use in safety critical applications, like autonomous driving and medical systems. %Many methods have been proposed for generating such adversarial perturbations.
Adversarial inputs usually produce perturbations imperceptible to humans, but subvert learning systems. Depending on how much information is available, we can divide attackers into \textit{white box} or \textit{black box} attacks. If the attacker has full access to the internal parameters of the model, it is termed as a white box attacker. In the case the attacker has access to the output label only, it is called a black box attacker. %Black box attacks can further be \textit{label only} or \textit{score only}. 
It is possible to successfully attack neural networks in both black box \citep{black_box_practical, black_box_hop_skip_jump_attack, black_box_limited_attacks, black_box_square_attack} and white box setting \citep{white_box_carlini_wagner, pmlr-v80-athalye18a, white_box_pgd, white_box_fgsm}. The presence of adversarial perturbations motivated training with robustness in mind. This involves adding counterexamples to the classifiers during an \textit{adversarial training} process \citep{defense_madry2019deep}. While this has had a positive impact on robustness, there is significant room for improvement.

%An adversarial data point is typically close to a original datapoint, but flips the output of the classifier. Pixel level perturbations should not flip the \textit{true} label of an image because small changes in pixel values are often imperceptible to human vision. 

% A first insight of how to be robust to small imperceptible changes is that the visual cortex prioritises integration of information across larger receptive fields above high resolution processing. Visual acuity in humans is a measure of the sharpness of vision, the ability to discern objects at a distance.
% During early childhood development poor retinal acuity is surprisingly common  \citep{visual_acuity}, causing blurry vision.  This allows the visual cortex to learn processing strategies over larger receptive fields. Deep neural networks are functions which work on high-resolution images, creating non-smooth decision boundaries. Thus, we propose a pre-processing step which lowers the resolution slightly. We group pixels using locally coherent properties into \textit{image segments}, and replace them with the color of the segment. 

% The second insight comes from studies relating to face recognition as a visual skill. Face recognition often functions in an "experience-expectant" fashion \citep{face_recognition_exp_1, face_recognition_exp_2}. While this might be different from general object recognition \citep{FARAH1996181}, we use this insight to guide our algorithm. We explicitly model the experience as \textit{memories}, and process test datapoints depending on their similarity to these memories. This allows the classifier to switch operating regions. If a test point is too dissimilar from a previously seen object, it is classified  as an unknown. %At the same time, allowing for semantic preserving transformation to increase the accuracy of the classifier. 

\textbf{Contributions: }
1. We propose a way to incorporate prototypes as \textit{memories}. The first step in our
algorithm is to pick the representative samples of the dataset by analyzing the
\textit{commonalities}. These representative samples are used to describe 
different groups in the data. We learn a different classifier for each such sub-group.
2. Image transforms preserving semantics can be conveniently incorporated into our learning system. We test the robustness against rotational and shift perturbations.
3. We evaluate black box robustness against adversarial pixel level perturbations. Additionally, we can use memories as anchors to correct for random rotation or shift.



\textbf{Roadmap: }   
% \includegraphics[height = 8cm, width = 13cm]{Figures/memory_classifier.png}
We begin with a brief description of a \mc\ in Section \ref{sec:memory_classifier}. Where we explain memory classifiers at a high level, and prove under what condition the results generalize better.
Following which we describe the learning algorithm specialized to images in Section \ref{sec:memory_classifier_for_images}. Followed by experimental results, Section \ref{sec:experiments}, related work Section \ref{sec:related_work}, and conclusive remarks in Section \ref{sec:conclusions}.  

\begin{figure*}[t]
    \centering
    \includegraphics[height = 9cm, width = 17cm]{Figures/overall_diagram.png}
    \caption{\footnotesize{\Mc: The decision function of a memory classifier is broken up into two distinct stages. At first the test image gets mapped to a \emph{memory} image using a \emph{matching algorithm}. Once matched the final decision is issued by a SOTA classifier such as a Resnet. The \emph{matching algorithm} uses a context specific information for the problem to map to a memory. The context specific information causes a shift in the distribution of the samples that a memory picks. }}
    \label{fig:memory_classifier}
\end{figure*}


==> memory_classifiers_for_images.tex <==
\section{Memory Classifiers for Images}
\label{sec:memory_classifier_for_images}

We refer the readers to Figure \ref{fig:memory_classifier} as an overview. 
The test input is first mapped to a candidate memory, and then depending on the match it chooses a different classifier.  In this section we explain the details of the match computation and classification workflow  adopted in the case of the images as inputs. Big leaps have been made in the field of computer vision using with our ability to train complex DNNs. But, they come with brittleness which is a big roadblock to wide scale adoption. Not only in the form of directed white box attacks, but from random and seemingly benign distribution shifts as well. \todo{cite the papers}.

% We assume that an image \im is 3-d array of size $l \times l \times 3$, such that $\ima(p,q, .) \in (0, 1), $ and $0 \leq p,q < l$. As a pre-processing step we partition a given image into different segments, or groups of pixels depending on the color value. We use an off the shelf k-means clustering algorithm to group the pixels, and replace the pixel value with the cluster center. We denote this transform by $\ima_s = \seg(\ima)$. There could be potentially different ways of segmenting an image that one can explore, but we stick to clustering for simplicity.

\subsection{Distance between Images}

We begin with an anecdote. It is typically hard for human vision to be able to tell the difference two closely related QR codes but a machine can do it with ease. However, it is relatively easy to perturb an image of a cat, in order to make a DNN label it as a dog. But humans cannot be fooled by such alterations at pixel level. The first insight of how to be robust to such imperceptible changes comes from studies relating to the visual cortex. The human brain prioritises integration of information across larger receptive fields above high resolution processing. Visual acuity in humans is a measure of the sharpness of vision, the ability to discern objects at a distance. During early childhood development poor retinal acuity is surprisingly common  \citep{visual_acuity}, causing blurry vision.  This allows the visual cortex to learn processing strategies over larger receptive fields. Deep neural networks are functions which work on high-resolution images, creating non-smooth decision boundaries.

The second insight comes from studies relating to face recognition as a visual skill. Face recognition often functions in an "experience-expectant" fashion \citep{face_recognition_exp_1, face_recognition_exp_2}. While this might be different from general object recognition \citep{FARAH1996181}, we use this insight to guide our algorithm. We explicitly model the \emph{experience} by storing sample points. Afterwards, we process test datapoints depending on their similarity to these samples. This permits the classifier to restrict classification to images only when they are within boundary of similarity. This feature allows for out-of-distribution detection. Imagine a classifier for face recognition systems. It should only issue a classification when the image looks somewhat like a human face, but should refrain from classifying anything in all other cases. DNNs are vulnerable to such out-of-distribution(OOD) attacks. This is a realm of on-going research in being able to detect such pitfalls due to distribution shifts. \todo{cite OOD papers}

To bridge these gaps discussed above, we delve into a rich and existing body of work broadly referred to as digital image processing. Digital image processing \todo{cite a book} offers us tools and techniques to capture the macro properties in an image. These higher level properties of an image, could then be potentially translated to answer why two images look similar. For instance, given a pair of images both containing a traffic "STOP" sign, we could measure the number of red pixels in the images to compute an affinity measure between them. Binning different training samples induces an implicit distribution shift, which can potentially lead to an improvement in robustness properties of the overall classifier.

Let us assume we are given two images $\ima_1$ and $\ima_2$, and we wish to compute a similarity score between them. 
The function $\s ( \ima_1, \ima_2) \rightarrow [0,1]$, could be potentially a manually designed modest classifier as well.
For example, a decision tree based on macro level image properties. Where $\s(\ima_1, \ima_2) = 1 $, only when the classifier maps them to the same class. This might end up skewing the class-distribution for the following classifier. But there are methods like class-balancing, and loss re-weighting to counter this effect. \todo{cite a book for this.}



